Dupin: A Parallel Framework for Densest Subgraph Discovery in Fraud Detection on Massive Graphs (Technical Report)

Detecting fraudulent activities in financial and e-commerce transaction networks is crucial. One effective method for this is Densest Subgraph Discovery (DSD). However, deploying DSD methods in production systems faces substantial scalability challenges due to the predominantly sequential nature of existing methods, which impedes their ability to handle large-scale transaction networks and results in significant detection delays. To address these challenges, we introduce Dupin, a novel parallel processing framework designed for efficient DSD processing in billion-scale graphs. Dupin is powered by a processing engine that exploits the unique properties of the peeling process, with theoretical guarantees on detection quality and efficiency. Dupin provides userfriendly APIs for flexible customization of DSD objectives and ensures robust adaptability to diverse fraud detection scenarios. Empirical evaluations demonstrate that Dupin consistently outperforms several existing DSD methods, achieving performance improvements of up to 100 times compared to traditional approaches. On billion-scale graphs, Dupin demonstrates the potential to enhance the prevention of fraudulent transactions from 45% to 94.5% and reduces density error from 30% to below 5%, as supported by our experimental results. These findings highlight the effectiveness of Dupin in real-world applications, ensuring both speed and accuracy in fraud detection.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> _1-revision.tex <==
\begin{center}
  {\fontsize{18pt}{16.8pt}\selectfont \textbf{Revision Response}}
\end{center}
\begin{multicols}{2}

\renewcommand{\thefigure}{\Alph{figure}} % Change Font of Figure numbering.

\noindent Dear Reviewers:

We sincerely appreciate your constructive feedback for us to improve the quality of our work. We have made substantial changes to address your comments. Changes are highlighted in \textcolor{blue}{\textbf{blue}}. In the following, we provide a summary of the changes in this revision.


\vspace{-0.5em}
\section*{SUMMARY OF CHANGES}

\begin{enumerate}[leftmargin=5mm]
    \item \stitle{Clarifying Contributions and Comparisons:} We compare our approach with \Spade{}/\Spade{}+ and clarify differences (\hyperref[com:R2O1]{R2-O1}). We also restructure the introduction to integrate real-world scenarios and highlight key contributions (\hyperref[com:R4O1]{R4-O1}, \hyperref[com:R3O1]{R3-O1}). 
    \item \stitle{Framework \& API Details:} We restore an API listing to show how density metrics are defined and clarify that they are configured, not dynamically swapped (\hyperref[com:R2O2]{R2-O2}).
    \item \stitle{Parallel Execution:} We explicitly detail parallel operations (\hyperref[com:R2O3]{R2-O3}) in our algorithms and add a figure showing CPU utilization under multiple threads (\hyperref[com:R4O2]{R4-O2}).
    \item \stitle{Improved Presentation \& Experiments:} We refine key definitions, provide proofs in the appendix of~\cite{dupin2024} (\hyperref[com:R2M1]{R2-M1}, \hyperref[com:R4M6]{R4-M6}), add a figure plotting accuracy vs. runtime (\hyperref[com:R4O3]{R4-O3}), and integrate motivating examples directly into the introduction (\hyperref[com:R4M1]{R4-M1}).
\end{enumerate}

\smallskip

Due to space constraints, we have prepared a Supplementary File for this paper~\cite{dupin2024}, which includes additional materials such as extended experiments and detailed proofs. We have updated the Supplementary File in the CMT system. In case of access issues, it is also available at: \href{https://drive.google.com/drive/folders/1TJxwFm7b_Q5ihyyP4ZOaGKMBvJscEfbg?usp=sharing}{\stitle{https://drive.google.com/drive/folders/1TJxwFm7b\_Q5ihyyP4Z OaGKMBvJscEfbg?usp=sharing}}.


% Due to space constraints, we have prepared a complete version of the paper as a technical report~\cite{dupin2024}, which includes additional materials such as extended experiments and detailed proofs. The technical report is available at: \href{https://drive.google.com/drive/folders/1TJxwFm7b_Q5ihyyP4ZOaGKMBvJscEfbg?usp=sharing}{\stitle{https://drive.google.com/drive/folders/1TJxwFm7b\_Q5ihyyP4Z OaGKMBvJscEfbg?usp=sharing}}
% %\href{https://anonymous.4open.science/api/repo/Dupin-IMPL-3DE6/file/Dupin_SIGMOD_Revision_TR.pdf}{\stitle{https://anonymous.4open.science/api/repo/Dupin-IMPL-3DE6/file/Dupin_SIGMOD_Revision_TR.pdf}}

\section*{RESPONSE TO REVIEWER 2}

\rev[R2O1]{\phantomsection
\label{com:R2O1}There is quite an overlap between the concepts and presentation of this paper and the \Spade{}+ paper~\cite{jiang2024spade+}. However, the comparisons are done against \Spade{} (no edge deletions). If this paper is a parallel version of \Spade{} or \Spade{}+, this should be clarified. As is, several statements in this paper's motivation simply present faults in other approaches but leave the substantiating of these faults somewhat incomplete. Was the claim that \Spade{} takes 198 seconds per batch evaluated with the same machine as the experimental section (Xeon X5650)? That machine is 14 years old, \ie{} it has a fraction of the memory bandwidth and processing capacity of what even a modest, more recent server has. Put differently, the results presented are most likely outdated.}
%
\res{Thank you for your detailed and insightful feedback. We outline our revisions below.\\
\stitle{1. Rewriting the Preliminary Algorithm.} The section on the preliminary algorithm is rewritten to improve its presentation as a background discussion. We add additional citations~\cite{tsourakakis2015k,hooi2016fraudar,bahmani2012densest,chekuri2022densest,jiang2023spade,jiang2024spade+} to ensure proper attribution and context, differentiating our contributions from those of \Spade{} and \Spade{}+ more clearly. \\
\stitle{2. Clarifying the Relationship with \Spade{}/\Spade{}+.} We clarify in the revised paper that \Dupin{} is not a parallel version of \Spade{} or \Spade{}+ in Section~\ref{sec:intro}. \Spade{} and \Spade{}+ are \textbf{the incremental version} of the peeling algorithm, while \Dupin{} represents \textbf{the parallel version} of the peeling algorithm. These are two distinct approaches for dense subgraph computation in large-scale graphs. For $G\oplus\Delta G$, \Spade{} incrementally maintains dense subgraphs on $G$ for a given $\Delta G$. However, when $\Delta G$ is large, \Spade{} incurs significant overhead and can accumulate errors for metrics like $\Fraudar{}$ (Figure~\ref{fig:spade-heavy-time}). In contrast, \Dupin{} computes dense subgraphs from scratch in parallel directly on $G\oplus\Delta G$, avoiding these issues. This makes \Dupin{} and \Spade{} orthogonal in their approaches. We note that \Spade{}+ differs from \Spade{} solely in its approach to handling edge deletions. In our experiments, we utilized the latest codebase made available by the \Spade{}/\Spade{}+ authors, and this has been explicitly mentioned in the revised paper. \\
\stitle{3. Redesigning the System Architecture.} We have redesigned the architecture diagram (Figure~\ref{fig:architecture}) to provide a clearer illustration of \Dupin{}'s components. A detailed description accompanies the new diagram to help readers understand the system's functionality.\\
\stitle{4. Hardware Evaluation.} 
\begin{enumerate}[leftmargin=*]
    \item We clarify that the hardware (Xeon X5650) used in our submission was selected to ensure a fair comparison with the setup reported in \Spade{}’s original work in Section~\ref{subsec:setup}.
    \item To address concerns regarding hardware, we performed additional tests on a modern EPYC 7742 processor. The results, detailed in Table~\ref{tab:performance-comparison}, indicate that \Dupin{} achieves a 1.91–2.25$\times$ speedup on EPYC 7742 compared to Xeon X5650, while \Spade{} attains only a 1.08–1.15$\times$ speedup. \Dupin{}'s performance scales nearly linearly with the number of cores, efficiently leveraging the memory bandwidth and parallelism of contemporary hardware. In contrast, \Spade{}'s largely sequential design limits its scalability. These findings are included in the appendix of~\cite{dupin2024} to provide a comprehensive comparison of the evaluated systems.
\end{enumerate}
} 



\smallskip




\rev[R2O2]{\phantomsection
\label{com:R2O2}One of the main claims of the paper is that density functions could be swapped---dynamically?---and Fig~\ref{fig:architecture} seems to indicate that these functions can be described via an API. However, the API was never presented, nor was the ability to encode new density functions discussed. The example in Listing~\ref{lst:fraudar} shows that entire functions could be passed into the framework. If this is what dynamic density function means, the paper may be overclaiming.}
%
\res{
\stitle{1. Clarifying the Density Metric Selection.} In the revised paper, we clarify that \Dupin{} allows moderators to select density metrics, which are defined by developers, based on specific business requirements, rather than enabling dynamic swapping of density functions at runtime. For example, in fraud detection, a density metric that weights transaction amounts can better highlight collusion patterns—such as frequent high-value or consistent transactions indicative of coupon or rebate abuse—compared to fixed scoring functions. This discussion has been expanded to emphasize \Dupin{}’s flexibility in tailoring density metrics to particular use cases.\\
\stitle{2. Restoring API Details in the Paper.} We have reinstated the API definitions in Listing~\ref{lst:dupin_api} as a dedicated listing in the revised paper. This inclusion provides a clear and complete view of how density metrics can be defined and integrated into the framework. We use $\Fraudar{}$ as an example in Listing~\ref{lst:fraudar} to demonstrate how a density metric can be defined in \Dupin{}. For other density metrics, implementation details are provided in Appendix~\ref{appendix:implementation} of~\cite{dupin2024}. \\
}


\rev[R2O3]{\phantomsection
\label{com:R2O3}Another claim of the paper is parallel execution, presumably of the peeling function. Instead, what is presented in Alg~\ref{algo:peeling:batch} is akin to a batching. Fig~\ref{fig:parallel} (as Fig~\ref{fig:peeling}) shows a very convenient case in which the weight increases with the peeling order, which seems improbable in real graphs. (See additional details below.) Therefore, it is unclear how multi-threaded parallelism, which appears in the experiments somewhat suddenly, is woven into the algorithms.}
%
\res{\stitle{1. Adding Details on Parallel Execution.} We expand the discussion of parallel execution in the paper. Specifically, we modify Algorithm~\ref{algo:peeling:batch}, ~\ref{algo:peel2}, ~\ref{algo:peel3} to explicitly highlight the parallel operations, demonstrating that our algorithm is a parallel peeling algorithm rather than simple batching. For instance, we showcase the parallel computation of peeling weights for multiple vertices, the parallel evaluation of whether vertices should be peeled, and other parallel steps in the algorithm. \\
\stitle{2. Clarifying Figure~\ref{fig:peeling} and Figure~\ref{fig:parallel}.} Figure~\ref{fig:peeling} and Figure~\ref{fig:parallel} do not show monotonic weight increases with the peeling order. For example, Figure~\ref{fig:peeling} returns the densest structure in Iteration $2$, and Figure~\ref{fig:parallel} identifies the densest subgraph in Iteration 1. We clarify this in Example~\ref{example:parallel} and Example~\ref{example:parallel:clique} to explain the inherent non-monotonicity of the peeling process.\\
}

\rev[R2M1]{\phantomsection
\label{com:R2M1}Reference~\cite{goldberg1984finding}, which is important in the paper, is incomplete. Add the journal in which it was published.
}
%
\res{Reference~\cite{goldberg1984finding} is a technical report. We have updated it to include the complete details as follows: 

\noindent \textit{A. V. Goldberg. Finding a maximum density subgraph. Technical report, University of California, Berkeley, USA, 1984. EECS Technical Memorandum Series.} \\}

\rev[R2M2]{\phantomsection
\label{com:R2M2}It is unclear from example~\ref{exp:2.1} what would happen with the sequential algorithm if the weights did not increase along the peeling order. Moreover, it is also unclear why Theorem~\ref{thm:3ppr_cli} holds. Why is the intuition that allows one to state that the suspiciousness of the result of the sequential algorithm is twice as large as the optimal vertex set?}
%
\res{
\stitle{1. Clarifying the Behavior of the Sequential Peeling Algorithm.} In the revised paper, we clarify that the sequential peeling algorithm is designed with a 2-approximation guarantee when density metrics such as \(\DENG\), \(\DENGW\), and \(\Fraudar\) are used. Specifically, these guarantees ensure that the density (and, hence, the suspiciousness) of the subgraph returned by the sequential algorithm is at least half of that of the optimal subgraph—that is, the optimal subgraph’s suspiciousness cannot exceed twice the value obtained by the sequential algorithm. We further explain in Examples~\ref{example:parallel} and~\ref{example:parallel:clique} that although the peeling weight of each vertex decreases during the iterative peeling process, there is an inherent non-monotonicity in the density along the peeling order, which does not affect the overall approximation guarantee.

\stitle{2. Proof for Theorem~\ref{thm:3ppr_cli}.} A formal proof of Theorem~\ref{thm:3ppr_cli} is included in the appendix (see Appendix~\ref{subsec:appendix:proof} of~\cite{dupin2024}).\\
}


\rev[R2M3]{\phantomsection
\label{com:R2M3}Section $3.1$ can use a practical example of why a dense graph implies customer-merchant collusion rather than a popular item being sold by the latter to the formers.}
%
\res{To address the concern, we have revised the paper to incorporate a practical example illustrating why a dense subgraph is more indicative of customer-merchant collusion than merely a popular item being sold. Specifically, we have introduced an industry use case in collaboration with $\Grab$ (anonymized for review). We have added Figure~\ref{fig:intro:example} to visually illustrate this distinction and moved the discussion to the Introduction (Section~\ref{sec:intro}) to provide a more compelling contextual motivation for the problem.\\}


\section*{RESPONSE TO REVIEWER 3}
\rev[R3O1]{\phantomsection
\label{com:R3O1}Compared to previous work, what are the main novelties in the algorithms of the new approach? You discuss them throughout the paper, but, it would be useful to collect them in a table or list.}
%
\res{Thank you for your suggestion. We create Table~\ref{tab:algorithm-comparison} summarizing the algorithms compared in our experiments across key dimensions: Density Metric Support, Parallelizability, Weighted Graph Support, and Pruning Support. This should clearly highlight the distinctions and novelties of our approach. We place this table in Section~\ref{sec:intro} to give readers a clear overview of how our work differs from existing methods right from the beginning. Entries marked with (*) indicate methods that support only a single density metric and require modifications to the codebase for performance testing.
}

\section*{RESPONSE TO REVIEWER 4}
\rev[R4O1]{\phantomsection
\label{com:R4O1} I would suggest to rewrite the introduction and move Section~$3.1$ to essentially be the intro. Section~$3.1$ describes well why \DDS{} is important for fraud detection and how it works in a real-world setting. Currently the introduction is somewhat abstract and does not motivate the problem that well.}
%
\res{Thank you for the suggestion. We rewrite the introduction to provide a clearer and more compelling motivation for the problem with concrete examples. Key points from Section~$3.1$ are integrated to explain why \DDS{} is critical for fraud detection and how it addresses real-world challenges. \\
We incorporate Figure~\ref{fig:intro:example} to illustrate the significance of \DDS{} in fraud detection. Specifically, detecting dense subgraphs is vital for uncovering suspicious activities, such as Customer-Merchant Collusion, where clusters of customers and merchants repeatedly interact through anomalous transaction patterns, potentially indicating the abuse of discounts or coupons.\\}

\rev[R4O2]{\phantomsection
\label{com:R4O2}In the experiments, it would be good to have a figure that plots the utilization when using multiple threads.}
%
\res{We have addressed the comment by adding a new figure that plots CPU utilization when using multiple threads. Figure~\ref{fig:breakdown:main} has been added to the revised paper. It shows CPU utilization for the parallel algorithms on the \texttt{soc} and \texttt{sk} datasets with respect to the $\DENG$ density metric. As the number of threads increases from $2$ to $64$, both \GBBS{} and \ALENEX{} exhibit a faster growth in stall rates compared to \Dupin{}, demonstrating the superior scalability of \Dupin{}. For the $\DENGW$ and $\Fraudar$ density metrics, and for the other datasets, similar plots are provided in Figures~\ref{fig:breakdown:appendix}--\ref{fig:breakdown:appendix:fd} in Appendix~\ref{appendix:exp} of~\cite{dupin2024}.\\ }

\rev[R4O3]{\phantomsection
\label{com:R4O3}A more in-depth comparison on the tradeoff between accuracy and speed. For example, there should be a figure that plots accuracy (so best density) \wrt runtime and compare this with the points that other systems achieve.}
%
\res{We have addressed the comment by adding a new figure that plots accuracy (i.e., best density achieved) versus runtime, offering an in-depth view of the tradeoff between accuracy and speed. Figure~\ref{fig:DG:runtime:density} in the experimental section shows this tradeoff for the $\DENG$ metric on the \texttt{soc} and \texttt{sk} datasets, and it compares the performance points of our approach with those of other systems. For the $\DENGW$ and $\Fraudar$ density metrics, as well as for other datasets, we have provided similar plots in Figures~\ref{fig:DG:runtime:density:appendix}--\ref{fig:FD:runtime:density:appendix} in Appendix~\ref{appendix:exp} of~\cite{dupin2024}.\\}

\rev[R4M1]{\phantomsection
\label{com:R4M1}Why is the \DDS{} problem important for fraud detection? It would be useful to motivate this more concretely, or at least explain some scenarios where we want to do \DDS{} instead of something else.}
%
\res{We add concrete examples to explain why the \DDS{} problem is important for fraud detection in Section~\ref{sec:intro} Introduction. For instance, \DDS{} helps identify tightly connected groups indicative of suspicious activities, such as customer-merchant collusion or coordinated account takeovers. These scenarios require detecting dense subgraphs to pinpoint fraud patterns that are not easily captured.\\}

\rev[R4M2]{\phantomsection
\label{com:R4M2}I do not understand what Figure~\ref{fig:heavy} depicts. Please mention what \Spade{} is.}
%
\res{
We have revised the description of Figure~\ref{fig:heavy} in the manuscript to clarify its purpose and to introduce \Spade{} as an incremental algorithm for maintaining dense subgraphs in dynamic graphs. Figure~\ref{fig:heavy} is intended to demonstrate that practical fraud detection in real-world settings continues to face critical efficiency limitations. We use the state-of-the-art incremental algorithm \Spade{}~\cite{jiang2023spade} as an example. In the revised manuscript (Section~\ref{sec:intro}), we now explain:

\begin{itemize}
    \item \textbf{Inefficient Incremental Updates.} Current incremental algorithms often fail to scale to billion-edge graphs with high transaction rates. For example, consider the state-of-the-art incremental algorithm \Spade{}~\cite{jiang2023spade} (Figure~\ref{fig:spade-heavy-time}), where the vertical axis represents the Device Activities Count (i.e., the number of new edges generated per minute) and the gray area indicates System Heavy Time. \Spade{} can process approximately \(2.65 \times 10^5\) edge updates per minute, which is insufficient to handle scenarios with high transaction volumes. Moreover, these methods often assume static edge weights, even though newly inserted edges can alter the weights of existing edges. For example, the cumulative density error of~\cite{jiang2023spade} can exceed 15\% in a single day (Figure~\ref{fig:density-comparison}).
\end{itemize}

This revision clarifies that Figure~\ref{fig:heavy} highlights the efficiency challenges in practical fraud detection and demonstrates these challenges using \Spade{} as a representative example. \\
}


\rev[R4M3]{\phantomsection
\label{com:R4M3}Section~\ref{subsec:preliminary}: the graph is directed on undirected?}
%
\res{Dupin supports both directed and undirected graphs, We make it clear in Section~\ref{subsec:preliminary}. \\}

\rev[R4M4]{\phantomsection
\label{com:R4M4}Why is the \TDS{} metric captured by Equation~\ref{eq:density}? This is not obvious at all. Same for the \KCDS metric.}
%
\res{We provide detailed formulations and explanations for the \TDS{} and \KCDS{} metrics in Section~\ref{subsec:preliminary}, showing how they are captured by Equation~\ref{eq:density}.\\}

\rev[R4M5]{\phantomsection
\label{com:R4M5}Section~\ref{subsec:SPA}: how is the peeling weight used in Algorithm~\ref{algo:peeling}? This is mentioned and then not used afterwards.}
%
\res{We have revised Algorithm~\ref{algo:peeling} to show the role of the peeling weight in selecting which vertex to remove at each iteration. In each iteration, the vertex \(u_i\) with the smallest peeling weight is removed from the current subset \(S_{i-1}\) to form \(S_i\). The peeling weight is therefore directly used in the vertex selection process.\\}

\rev[R4M6]{\phantomsection
\label{com:R4M6}Theorem~\ref{thm:3ppr_cli}: it would be nice to be able to see this proof in some appendix or additional document.}
%
\res{We have added the complete proof of Theorem~\ref{thm:3ppr_cli} in Appendix~\ref{subsec:appendix:proof} of~\cite{dupin2024} to provide the necessary justification and clarity.\\}

\rev[R4M7]{\phantomsection
\label{com:R4M7}Section~$3.1$: this section is great, and I would actually suggest that it should go to the introduction to concretely motivate this paper.}
%
\res{Thank you for the suggestion. We integrate the key points from Section~$3.1$ into the Introduction (Section~\ref{sec:intro}) to provide a more concrete motivation for the paper and engage readers early on.\\}

\rev[R4M8]{\phantomsection
\label{com:R4M8}Property~\ref{property:parallelization}: what does support mean here? Does it mean that it comes with theoretical guarantees? Or just that the system will run but may not guarantee anything?}
%
\res{"Support" in this context means that the system provides theoretical guarantees. We revise the description to clarify this.\\}

\rev[R4M9]{\phantomsection
\label{com:R4M9}Lemma~\ref{lemma:finite}: Define \( R \) for the lemma.}
%
\res{We define \( R \) in Lemma~\ref{lemma:finite} as the upper bound on the number of rounds required for the peeling.\\}

\rev[R4M10]{\phantomsection
\label{com:R4M10}Tables~\ref{tab:effectiveness-deng}, ~\ref{tab:effectiveness-tds}: what are the numbers in these tables?}
%
\res{We update the captions for Tables~\ref{tab:effectiveness-deng} and~\ref{tab:effectiveness-tds} to clearly indicate that the numbers represent density values, ensuring readers understand the content of the tables.}

\end{multicols}

==> listing_style.tex <==
\usepackage{listings}
\DeclareCaptionLabelFormat{listings}{\textbf{Figure #2}}
\captionsetup[lstlisting]{labelformat=listings}

\lstdefinestyle{mystyle}{
    language=C,
    basicstyle=\small\ttfamily,
    keywordstyle=\color{red},      % Color of keywords
    commentstyle=\color{green},    % Color of comments
    stringstyle=\color{black},       % Color of strings
    numbers=left,
    numberstyle=\tiny\color{gray}, % Color of line numbers
    frame=single,
    breaklines=true,
    captionpos=b,
    caption=Example Python Code,
    label=lst:pythoncode,
    morekeywords={bool},
    moredelim=[is][\color{blue}]{![}{!]},
    moredelim=[is][\color{green}]{@[}{@]},
}

\definecolor{myblue}{RGB}{0,0,255}
\definecolor{mygreen}{RGB}{0,128,0}
\definecolor{myred}{RGB}{255,0,0}
\definecolor{mygray}{RGB}{128,128,128}

\lstdefinestyle{mystyle2}{
    language=Python,
    basicstyle=\small\ttfamily,
    keywordstyle=\color{myblue},
    commentstyle=\color{mygreen},
    stringstyle=\color{myred},
    numbers=left,
    numberstyle=\tiny\color{mygray},
    frame=single,
    breaklines=true,
    captionpos=b,
    caption=Example Python Code,
    label=lst:pythoncode,
}







